Diverse Image Captioning with Grounded Style

Stylized image captioning as presented in prior work aims to generate captions that reflect characteristics beyond a factual description of the scene composition, such as sentiments. Such prior work relies on given sentiment identifiers, which are used to express a certain global style in the caption, e.g. positive or negative, however without taking into account the stylistic content of the visual scene. To address this shortcoming, we first analyze the limitations of current stylized captioning datasets and propose COCO attribute-based augmentations to obtain varied stylized captions from COCO annotations. Furthermore, we encode the stylized information in the latent space of a Variational Autoencoder; specifically, we leverage extracted image attributes to explicitly structure its sequential latent space according to different localized style characteristics. Our experiments on the Senticap and COCO datasets show the ability of our approach to generate accurate captions with diversity in styles that are grounded in the image.

==> Images/methods_model_arch.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,303); %set diagram left start at 0, and has height of 303
%Straight Lines [id:da6419814995930448] 
\draw    (441.84,234.11) -- (441.84,188.67) ;
\draw [shift={(441.84,185.67)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da17981880196363398] 
\draw    (461.67,184.17) -- (461.67,170.17) ;
\draw [shift={(461.67,167.17)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da4532907254605869] 
\draw    (498.75,174.37) -- (503.75,174.37) -- (503.75,150.88) ;
\draw [shift={(503.75,147.88)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da18358789340280735] 
\draw    (407.01,119.56) -- (407.01,105.99) ;
\draw [shift={(407.01,102.99)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da7557661735393177] 
\draw    (441.67,81.83) -- (441.82,58.12) ;
\draw [shift={(441.84,55.13)}, rotate = 450.36] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da4275990023213875] 
\draw    (459.56,132.53) -- (428.47,132.53) ;
\draw [shift={(425.47,132.53)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da9734068354786687] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (361.54,92.84) -- (381.6,92.84) ;
\draw [shift={(384.6,92.84)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da08738007532640124] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (360.54,173.84) -- (380.6,173.84) ;
\draw [shift={(383.6,173.84)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da6292479044142401] 
\draw    (360.54,212.2) -- (380.6,212.2) ;
\draw [shift={(383.6,212.2)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da7644256378625864] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (500.04,92.84) -- (520.1,92.84) ;
\draw [shift={(523.1,92.84)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da7536010529185087] 
\draw    (442,230.14) -- (405.6,230.14) -- (405.6,226) ;
\draw [shift={(405.6,223)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da8675911607495881] 
\draw    (405.6,201.67) -- (405.6,188.7) ;
\draw [shift={(405.6,185.7)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da30107539018056406] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (343.83,244.7) -- (363.89,244.7) ;
\draw [shift={(366.89,244.7)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da609316097723157] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (516.4,244.7) -- (536.46,244.7) ;
\draw [shift={(539.46,244.7)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da8128630334236409] 
\draw    (442,277.9) -- (442,258.7) ;
\draw [shift={(442,255.7)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da6687486044462898] 
\draw    (480.4,277.9) -- (480.4,266.8) -- (442,266.8) ;
%Straight Lines [id:da4817773107239971] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (442,277.9) -- (442,266.8) -- (403.6,266.8) -- (403.6,277.9) ;
%Straight Lines [id:da9757055805865936] 
\draw    (441.67,33.83) -- (441.67,22.22) ;
\draw [shift={(441.67,19.22)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;

% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (384.6,201.7) -- (426.6,201.7) -- (426.6,222.7) -- (384.6,222.7) -- cycle  ;
\draw (405.6,212.2) node  [font=\footnotesize] [align=left] {Attend};
% Text Node
\draw  [fill={rgb, 255:red, 185; green, 15; blue, 34 }  ,fill opacity=1 ]  (384.84,82.34) -- (498.84,82.34) -- (498.84,103.34) -- (384.84,103.34) -- cycle  ;
\draw (441.84,92.84) node  [font=\footnotesize] [align=left] {Language Decoder};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (415.84,33.93) -- (467.84,33.93) -- (467.84,54.93) -- (415.84,54.93) -- cycle  ;
\draw (441.84,44.43) node  [font=\footnotesize] [align=left] {Softmax};
% Text Node
\draw  [fill={rgb, 255:red, 185; green, 15; blue, 34 }  ,fill opacity=1 ]  (385.17,163.87) -- (498.17,163.87) -- (498.17,184.87) -- (385.17,184.87) -- cycle  ;
\draw (441.67,174.37) node  [font=\footnotesize] [align=left] {Language Encoder};
% Text Node
\draw (526.33,163.87) node  [font=\scriptsize] [align=left] {$\displaystyle \textcolor[rgb]{0.73,0.06,0.13}{h}\textcolor[rgb]{0.73,0.06,0.13}{^{encoder}_{t}}$};
% Text Node
\draw (442,284.2) node  [font=\footnotesize] [align=left] {$\displaystyle \overline{v}$};
% Text Node
\draw (467.61,224.2) node  [font=\footnotesize] [align=left] {$\displaystyle h^{attention}_{t}$};
% Text Node
\draw (415.1,192.87) node  [font=\footnotesize] [align=left] {$ $$\displaystyle \hat{v}_{t}$};
% Text Node
\draw (441.67,11.22) node  [font=\footnotesize] [align=left] {$\displaystyle y_{t}$};
% Text Node
\draw (480.4,284.2) node  [font=\footnotesize] [align=left] {$\displaystyle W_{e} \Pi _{t}$};
% Text Node
\draw (331.04,212.2) node  [font=\footnotesize] [align=left] {$\displaystyle \{v_{1} ,...,v_{k}\}$};
% Text Node
\draw  [fill={rgb, 255:red, 185; green, 15; blue, 34 }  ,fill opacity=1 ]  (454.34,117.53) -- (543.34,117.53) -- (543.34,147.53) -- (454.34,147.53) -- cycle  ;
\draw (498.84,132.53) node  [font=\footnotesize] [align=left] {$\displaystyle \mu _{\phi ,t} ,\ log\left( \sigma ^{2}_{\phi ,t}\right)$};
% Text Node
\draw (463.67,71.88) node  [font=\footnotesize,color={rgb, 255:red, 185; green, 15; blue, 34 }  ,opacity=1 ] [align=left] {$\displaystyle h^{decoder}_{t}$};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (367.43,234.2) -- (515.43,234.2) -- (515.43,255.2) -- (367.43,255.2) -- cycle  ;
\draw (441.43,244.7) node  [font=\footnotesize] [align=left] {Top-Down Attention LSTM};
% Text Node
\draw (544.47,92.84) node  [font=\footnotesize] [align=left] {$\displaystyle \textcolor[rgb]{0.73,0.06,0.13}{h}\textcolor[rgb]{0.73,0.06,0.13}{^{decoder}_{t}}$};
% Text Node
\draw (294.51,92.84) node  [font=\footnotesize] [align=left] {$\displaystyle \textcolor[rgb]{0,0,0}{h}\textcolor[rgb]{0,0,0}{^{attention}_{t}}\textcolor[rgb]{0,0,0}{,\ }\textcolor[rgb]{0,0,0}{\hat{v}}\textcolor[rgb]{0,0,0}{_{t}}\textcolor[rgb]{0,0,0}{,\ }\textcolor[rgb]{0.73,0.06,0.13}{c}\textcolor[rgb]{0.73,0.06,0.13}{(}\textcolor[rgb]{0.73,0.06,0.13}{I}\textcolor[rgb]{0.73,0.06,0.13}{)_{t}} ,\ \textcolor[rgb]{0.73,0.06,0.13}{h}\textcolor[rgb]{0.73,0.06,0.13}{^{decoder}_{t-1}}$};
% Text Node
\draw (327.44,174.44) node  [font=\footnotesize] [align=left] {$\displaystyle \textcolor[rgb]{0.73,0.06,0.13}{c}\textcolor[rgb]{0.73,0.06,0.13}{(}\textcolor[rgb]{0.73,0.06,0.13}{I}\textcolor[rgb]{0.73,0.06,0.13}{)_{t}} ,\ \textcolor[rgb]{0.73,0.06,0.13}{h}\textcolor[rgb]{0.73,0.06,0.13}{^{decoder}_{t-1}}$};
% Text Node
\draw (320.47,244.7) node  [font=\footnotesize] [align=left] {$\displaystyle h^{attention}_{t-1}$};
% Text Node
\draw (564.32,244.7) node  [font=\footnotesize] [align=left] {$\displaystyle h^{attention}_{t}$};
% Text Node
\draw (403.6,284.2) node  [font=\footnotesize] [align=left] {$\displaystyle \textcolor[rgb]{0.73,0.06,0.13}{h}\textcolor[rgb]{0.73,0.06,0.13}{^{decoder}_{t-1}}$};
% Text Node
\draw  [fill={rgb, 255:red, 185; green, 15; blue, 34 }  ,fill opacity=1 ]  (324.91,119.77) -- (432.91,119.77) -- (432.91,149.77) -- (324.91,149.77) -- cycle  ;
\draw (378.91,134.77) node  [font=\footnotesize] [align=left] {$\displaystyle \ z_{t} \sim \mathcal{N}\left( \mu _{\phi ,t} ,\ \sigma ^{2}_{\phi ,t}\right) \ $};
% Text Node
\draw (414.01,112.02) node  [font=\footnotesize] [align=left] {$\displaystyle \textcolor[rgb]{0.73,0.06,0.13}{z_{t}}$};


\end{tikzpicture}


==> Images/relwork_BUTD.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\centering

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,229); %set diagram left start at 0, and has height of 229

%Straight Lines [id:da938288443314668] 
\draw    (441.84,157.11) -- (441.84,111.67) ;
\draw [shift={(441.84,108.67)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da32397842049953607] 
\draw    (442.67,85.83) -- (442.82,62.12) ;
\draw [shift={(442.84,59.13)}, rotate = 450.36] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da4648919291515279] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (369.54,96.84) -- (389.6,96.84) ;
\draw [shift={(392.6,96.84)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da2339883827423187] 
\draw    (360.54,135.2) -- (380.6,135.2) ;
\draw [shift={(383.6,135.2)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da5436927153074607] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (493.04,96.84) -- (513.1,96.84) ;
\draw [shift={(516.1,96.84)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da11615337177974883] 
\draw    (442,153.14) -- (405.6,153.14) -- (405.6,149) ;
\draw [shift={(405.6,146)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da5172547896121543] 
\draw    (405.6,124.67) -- (405.6,111.7) ;
\draw [shift={(405.6,108.7)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da2533806964106097] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (343.83,167.7) -- (363.89,167.7) ;
\draw [shift={(366.89,167.7)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da5549087433246479] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (516.4,167.7) -- (536.46,167.7) ;
\draw [shift={(539.46,167.7)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da96886688381552] 
\draw    (442,200.9) -- (442,181.7) ;
\draw [shift={(442,178.7)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da3683954072451233] 
\draw    (480.4,200.9) -- (480.4,189.8) -- (442,189.8) ;
%Straight Lines [id:da8878996715235375] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (442,200.9) -- (442,189.8) -- (403.6,189.8) -- (403.6,200.9) ;
%Straight Lines [id:da8662221809745583] 
\draw    (442.67,37.83) -- (442.67,26.22) ;
\draw [shift={(442.67,23.22)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;

% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (384.6,124.7) -- (426.6,124.7) -- (426.6,145.7) -- (384.6,145.7) -- cycle  ;
\draw (405.6,135.2) node  [font=\footnotesize] [align=left] {Attend};
% Text Node
\draw    (393.51,87.01) -- (491.51,87.01) -- (491.51,108.01) -- (393.51,108.01) -- cycle  ;
\draw (442.51,97.51) node  [font=\footnotesize] [align=left] {Language LSTM};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (416.84,37.93) -- (468.84,37.93) -- (468.84,58.93) -- (416.84,58.93) -- cycle  ;
\draw (442.84,48.43) node  [font=\footnotesize] [align=left] {Softmax};
% Text Node
\draw (442,207.2) node  [font=\footnotesize] [align=left] {$\displaystyle \overline{v}$};
% Text Node
\draw (451.61,146.2) node  [font=\footnotesize] [align=left] {$\displaystyle h^{1}_{t}$};
% Text Node
\draw (413.1,114.87) node  [font=\footnotesize] [align=left] {$ $$\displaystyle \hat{v}_{t}$};
% Text Node
\draw (442.67,15.22) node  [font=\footnotesize] [align=left] {$\displaystyle x_{t}$};
% Text Node
\draw (480.4,207.2) node  [font=\footnotesize] [align=left] {$\displaystyle W_{e} \Pi _{t}$};
% Text Node
\draw (331.04,135.2) node  [font=\footnotesize] [align=left] {$\displaystyle \{v_{1} ,...,v_{k}\}$};
% Text Node
\draw (452.67,75.88) node  [font=\footnotesize,color={rgb, 255:red, 185; green, 15; blue, 34 }  ,opacity=1 ] [align=left] {$\displaystyle \textcolor[rgb]{0,0,0}{h^{2}_{t}}$};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (367.43,157.2) -- (515.43,157.2) -- (515.43,178.2) -- (367.43,178.2) -- cycle  ;
\draw (441.43,167.7) node  [font=\footnotesize] [align=left] {Top-Down Attention LSTM};
% Text Node
\draw (525.47,96.84) node  [font=\footnotesize] [align=left] {$\displaystyle \textcolor[rgb]{0,0,0}{h^{2}_{t}}$};
% Text Node
\draw (361.44,97.44) node  [font=\footnotesize] [align=left] {$\displaystyle \textcolor[rgb]{0,0,0}{h^{2}_{t-1}}$};
% Text Node
\draw (330.47,167.7) node  [font=\footnotesize] [align=left] {$\displaystyle h^{1}_{t-1}$};
% Text Node
\draw (548.32,167.7) node  [font=\footnotesize] [align=left] {$\displaystyle h^{1}_{t}$};
% Text Node
\draw (398.6,205.2) node  [font=\footnotesize] [align=left] {$\displaystyle \textcolor[rgb]{0,0,0}{h^{2}_{t-1}}$};


\end{tikzpicture}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tables/senticap_baseline_neg.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{\textbf{Method}}           & \multicolumn{1}{c}{\textbf{n}} & \multicolumn{1}{c}{\textbf{B1}} & \multicolumn{1}{c}{\textbf{B2}} & \multicolumn{1}{c}{\textbf{B3}} & \multicolumn{1}{c}{\textbf{B4}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{C}} & \multicolumn{1}{c}{\textbf{M}} \\ \midrule
Senticap,   Mathews et al. \cite{Mathews2015}           & 1 & 50.0                            & 31.2                            & 20.3                            & 13.1                            & 37.9                           & 61.8                           & 16.8                           \\
StyleNet, Gan   et al. \cite{Gan2017}*               & 1 & 43.7                            & -  & 10.6                            & -  & - & 36.6                           & 10.9                           \\
You et al.   \cite{You2018}                         & 1 & 52.2                            & 33.6                            & 22.2                            & 14.8                            & 39.8                           & 70.1                           & 17.1                           \\
Chen et al.   \cite{Chen2018b}                        & 1 & 50.3                            & 31.0                            & 20.1                            & 13.3                            & 38.0                           & 59.7                           & 16.2                           \\
Senti-Attend,   Nezami et al. \cite{Nezami2018}        & 1 & 58.6                            & 35.4                            & 22.3                            & 14.7                            & 45.7                           & 71.9 & 19.0\\
MSCap, Guo et   al. \cite{Guo2019}*                  & 1 & 45.5                            & -  & 15.4                            & -  & - & 51.6                           & 16.2                           \\
Attendgan,   Nezami et al. \cite{Nezami2019}           & 1 & 56.2                            & 34.1                            & 21.3                            & 13.6                            & 44.6                           & 64.1                           & 17.9                           \\
Memcap, Zhao   et al. \cite{Zhao2020}*                & 1 & 49.2                   & -                   & 18.1                   & -                   & -                  & 59.4                  & 15.7                  \\ \midrule
\textit{Karayil   et al. \cite{Karayil2019}}            & \textit{1}                     & \textit{57.0}                   & \textit{36.2}                   & \textit{23.4}                   & \textit{15.1}                   & \textit{44.5}                  & \textit{50.9}                  & \textit{19.9}                  \\
\textit{}      & \textit{10}                    & \textit{67.6}                   & \textit{46.3}                      & \textit{31.9}                   & \textit{21.9}                      & \textit{50.4}                     & \textit{68.8}                  & \textit{23.5}                  \\ \midrule
\multirow{4}{*}{\textbf{\textcolor{green}{Style}-SeqCVAE (ours)}} & \textbf{1}                     & \textbf{55.2}                   & \textbf{34.5}                   & \textbf{21.5}                   & \textbf{13.4}                   & \textbf{41.5}                  & \textbf{75.5}                  & \textbf{19.4}                  \\
               & \textbf{5}                     & \textbf{63.9}                   & \textbf{43.8}                   & \textbf{30.2}                   & \textbf{20.8}                   & \textbf{48.5}                  & \textbf{101.7}                 & \textbf{23.2}                  \\
               & \textbf{10}                    & \textbf{66.1}                   & \textbf{46.8}                   & \textbf{33.3}                   & \textbf{23.7}                   & \textbf{50.9}                  & \textbf{111.9}                 & \textbf{24.4}                  \\
               & \textbf{100}                   & \textbf{74.0}                   & \textbf{56.3}                   & \textbf{43.1}                   & \textbf{33.0}                   & \textbf{57.9}                  & \textbf{145.8}                 & \textbf{28.7}                  \\ \bottomrule
\end{tabular}
\caption{Top-1-Oracle scores on Senticap test split captions with negative sentiment.}
\label{tab:senticap_baseline_neg}

==> tables/senticap_baseline_pos.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}

\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{\textbf{Method}}           & \multicolumn{1}{c}{\textbf{n}} & \multicolumn{1}{c}{\textbf{B1}} & \multicolumn{1}{c}{\textbf{B2}} & \multicolumn{1}{c}{\textbf{B3}} & \multicolumn{1}{c}{\textbf{B4}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{C}} & \multicolumn{1}{c}{\textbf{M}} \\ \midrule
Senticap,   Mathews et al. \cite{Mathews2015}           & 1                              & 49.1                            & 29.1                            & 17.5                            & 10.8                            & 36.5                           & 54.4                           & 16.8                           \\
StyleNet, Gan   et al. \cite{Gan2017}*               & 1                              & 45.3                            & -                               & 12.1                            & -                               & -                              & 36.3                           & 12.1                           \\
You et al.   \cite{You2018}                         & 1                              & 51.2                            & 31.4                            & 19.4                            & 12.3                            & 38.6                           & 61.1                           & 17.2                           \\
Chen et al.   \cite{Chen2018b}                        & 1                              & 50.5                            & 30.8                            & 19.1                            & 12.1                            & 38.0                           & 60.0                           & 16.6                           \\
Senti-Attend,   Nezami et al. \cite{Nezami2018}        & 1                              & 57.6                            & 34.2                            & 20.5                            & 12.7                            & 45.1                           & 68.6                           & 18.9                           \\
MSCap, Guo et   al. \cite{Guo2019}*                  & 1                              & 46.9                            & -                               & 16.2                            & -                               & -                              & 55.3                           & 16.8                           \\
Attendgan,   Nezami et al. \cite{Nezami2019}           & 1                              & 56.9                            & 33.6                            & 20.3                            & 12.5                            & 44.3                           & 61.6                           & 18.8                           \\
Memcap, Zhao   et al. \cite{Zhao2020}*                & 1                              & 51.1                            & -                               & 17.0                            & -                               & -                              & 52.8                           & 16.6                           \\ \midrule
\textit{Karayil   et al. \cite{Karayil2019}}            & \textit{1}                     & \textit{54.7}                   & \textit{34.6}                   & \textit{22.0}                   & \textit{14.4}                   & \textit{41.8}                  & \textit{46.1}                  & \textit{18.5}                  \\
\textit{}                                   & \textit{10}                    & \textit{65.6}                   & \textit{43.9}                   & \textit{29.5}                   & \textit{20.2}                   & \textit{48.8}                  & \textit{63.1}                  & \textit{22.1}                  \\ \midrule
\multirow{4}{*}{\textbf{\textcolor{green}{Style}-SeqCVAE (ours)}} & \textbf{1}                     & \textbf{53.8}                   & \textbf{33.2}                   & \textbf{20.1}                   & \textbf{12.5}                   & \textbf{41.5}                  & \textbf{71.1}                  & \textbf{19.7}                  \\
                                            & \textbf{5}                     & \textbf{63.4}                   & \textbf{43.5}                   & \textbf{29.5}                   & \textbf{19.9}                   & \textbf{49.0}                  & \textbf{99.2}                 & \textbf{23.9}                  \\
                                            & \textbf{10}                    & \textbf{66.3}                   & \textbf{46.3}                   & \textbf{32.2}                   & \textbf{22.2}                   & \textbf{51.2}                  & \textbf{110.5}                 & \textbf{25.2}                  \\
                                            & \textbf{100}                   & \textbf{73.2}                   & \textbf{54.8}                   & \textbf{41.5}                   & \textbf{31.6}                   & \textbf{57.6}                  & \textbf{141.8}                 & \textbf{29.0}                  \\ \bottomrule
\end{tabular}
\caption{Top-1-Oracle scores on Senticap test split captions with positive sentiment: Performance according to each metric in comparison to work in the same domain. The column "n" is the number of generated samples. For the caption quality metrics, "B" is short for BLEU, "R" for ROUGE-L, "C" for CIDEr-D, "M" for METEOR. Approaches marked with "*" are multi style captioning approaches. Thus, a direct comparison is unfair, but for the sake of completeness they are included. Evaluation scores on a subset of the original test split are shown in italics. However, comparisons have shown that scores achieved on this subset are very similar to the full evaluation.}
\label{table:senticap_baseline_pos}

==> tables/swd_vs_glove.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htb]
\centering
\footnotesize
\begin{tabular}{ccrrrrr}
\hline
\multirow{2}{*}{\textbf{n}} & \multirow{2}{*}{\textbf{Method}}                                           & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{std}}} & \multicolumn{2}{c}{\textbf{n-gram Diversity}}                           & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Top-1\\ C\end{tabular}}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Avg\\ C\end{tabular}}}} \\ \cline{4-5}
                            &                                                                            & \multicolumn{1}{c}{}                              & \multicolumn{1}{c}{\textbf{Div-1}} & \multicolumn{1}{c}{\textbf{Div-2}} & \multicolumn{1}{c}{}                                                                            & \multicolumn{1}{c}{}                                                                          \\ \hline
                            & \multirow{2}{*}{Basic}                                                     & 1                                                 & 0.27                                  & 0.39                                  & 137.4                                                                                               & 78.3                                                                                             \\
                            &                                                                            & 2                                                 & 0.34                                  & 0.55                                  & 131.1                                                                                               & 61.6                                                                                             \\ \cline{2-7} 
20                          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textcolor{green}{Style}-SeqCVAE\\ SWD\end{tabular}} & 1                                                 & 0.27                               & 0.39                               & 137.9                                                                                           & 78.9                                                                                          \\
                            &                                                                            & 2                                                 & 0.34                               & 0.55                               & 130.5                                                                                           & 60.8                                                                                          \\ \cline{2-7} 
                            & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textcolor{green}{Style}-SeqCVAE\\ ATT\end{tabular}} & 1                                                 & 0.23                               & 0.31                               & 130.4                                                                                           & 84.9                                                                                          \\
                            &                                                                            & 2                                                 & 0.29                               & 0.43                               & 137.2                                                                                           & 75.2                                                                                          \\ \hline
                            & \multirow{2}{*}{Basic}                                                     & 1                                                 & 0.25                                  & 0.34                                  & 157.2                                                                                               & 78.5                                                                                             \\
                            &                                                                            & 2                                                 & 0.31                                  & 0.48                                  & 158.6                                                                                               & 61.5                                                                                             \\ \cline{2-7} 
100                         & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textcolor{green}{Style}-SeqCVAE\\ SWD\end{tabular}} & 1                                                 & 0.25                               & 0.34                          & 157.6                                                                                        & 78.8                                                                                             \\
                            &                                                                            & 2                                                 & 0.31                               & 0.48                                  & 157.9                                                                                               & 60.7                                                                                             \\ \cline{2-7} 
                            & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textcolor{green}{Style}-SeqCVAE\\ ATT\end{tabular}} & 1                                                 & 0.22                               & 0.28                               & 144.7                                                                                           & 85.0                                                                                          \\
                            &                                                                            & 2                                                 & 0.26                               & 0.37                               & 158.8                                                                                           & 75.0                                                                                          \\ \hline
\end{tabular}
\caption{Comparison of different latent space structuring approaches.}
\label{tab:my-table}
\end{table}

==> tables_backup/fact_capabilities.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
%\begin{table}[!htb]
%\centering
%\footnotesize
\caption{Evaluation of semantic accuracy.}
\begin{tabularx}{\textwidth}{@{}Xccccccccc@{}}
\toprule
    \multicolumn{1}{c}{\textbf{Method}}                                & \textbf{std} & \multicolumn{1}{c}{\textbf{B1}} & \multicolumn{1}{c}{\textbf{B2}} & \multicolumn{1}{c}{\textbf{B3}} & \multicolumn{1}{c}{\textbf{B4}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{C}} & \multicolumn{1}{c}{\textbf{M}} \\ \midrule
 Div-BS \cite{vijayakumar2016diverse}                                                            & --            & 83.7                            & 68.7                            & 53.8                            & 38.3                            & 65.3                           & 140.5                          & 53.7                           \\
                     AG-CVAE \cite{Wang2017}                                                           & --            & 83.4                            & 69.8                            & 57.3                            & 47.1                            & 63.8                           & 125.9                          & 30.9                           \\
                     POS \cite{deshpande2019fast}                                                               & --            & 87.4                            & 73.7                            & 59.3                            & 44.9                            & 67.8                           & 146.8                          & 36.5                           \\
                     Seq-CVAE \cite{Aneja2019}                                                         & --            & 87.0                            & 72.7                            & 59.1                            & 44.5                            & 67.1                           & 144.8                          & 35.6                           \\ \midrule
                     \multicolumn{1}{c}{\multirow{2}{*}{{Senti-SeqCVAE}}} & 1            & 84.2                   & 69.5                   & 56.0                   & 44.7                   & 63.4                  & 130.4               & 31.2                 \\
                     \multicolumn{1}{c}{}                                               & 2            & 86.6                   & 72.0                   & 58.8                   & 47.6                   & 65.9                  & 137.2                 & 32.8                  \\ \bottomrule
%\multirow{6}{*}{100} & Div-BS, Vijayakumar et al. \cite{vijayakumar2016diverse}                                                            & -            & 84.6                            & 69.8                            & 55.5                            & 40.2                            & 66.6                           & 144.8                          & 37.2                           \\
 %                    & AG-CVAE, Wang et al. \cite{Wang2017}                                                           & -            & 88.3                            & 76.7                            & 65.4                            & 55.7                            & 69.0                           & 151.7                          & 34.5                           \\
%                     & POS, Deshpande et al. \cite{deshpande2019fast}                                                               & -            & 92.1                            & 80.2                            & 68.9                            & 57.8                            & 73.9                           & 171.0                            & 42.3                           \\
 %                    & Seq-CVAE, Aneja et al. \cite{Aneja2019}                                                          & -            & 92.2                            & 80.3                            & 69.1                            & 57.5                            & 73.3                           & 169.5                          & 41.0                           \\ \cmidrule(l){2-10} 
 %                    & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{SeqSentiVAE   (ours)}}} & \textbf{1}            & \textbf{87.8}                   & \textbf{74.2}                   & \textbf{61.4}                   & \textbf{50.6}                   & \textbf{67.4}                  & \textbf{144.7}                 & \textbf{33.8}                  \\
 %                    & \multicolumn{1}{c}{}                                               & \textbf{2}            & \textbf{91.4}                   & \textbf{78.8}                   & \textbf{67.1}                   & \textbf{56.8}                   & \textbf{71.4}                  & \textbf{158.8}                 & \textbf{36.5}                  \\ \bottomrule
\end{tabularx}
\label{tab:results_fact_caps_acc}
%\end{table}

==> tables_backup/fact_diversity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
%\begin{table}[!htb]
%\centering
%\footnotesize
\caption{Caption diversity.}
\begin{tabularx}{\textwidth}{@{}Xccc@{}}
\toprule
 \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{std}}} & \multicolumn{2}{c}{\textbf{n-gram diversity}}  \\ \cmidrule{3-4} 
                           \multicolumn{1}{c}{}                                               & \multicolumn{1}{c}{}                              & \multicolumn{1}{c}{\textbf{Div-1}} & \multicolumn{1}{c}{\textbf{Div-2}} \\ \midrule
Div-BS \cite{vijayakumar2016diverse} & --  & 0.20  & 0.26 \\
AG-CVAE \cite{Wang2017}  & --  & 0.24 & 0.34 \\
POS \cite{deshpande2019fast}  & --   & 0.24   & 0.35\\
Seq-CVAE \cite{Aneja2019}    & --   & 0.25 & 0.54 \\ 
\midrule
\multicolumn{1}{c}{\multirow{2}{*}{{Senti-SeqCVAE}}} & 1 & 0.24 & 0.31\\
\multicolumn{1}{c}{} & 2  & 0.29    & 0.43        \\ \bottomrule
%\multirow{6}{*}{100}        & Div-BS, Vijayakumar et al. \cite{vijayakumar2016diverse}                                                             & -                                                 & 0.20                               & 0.25                               \\
%                            & AG-CVAE, Wang et al. \cite{Wang2017}                                                            & -                                                 & 0.23                               & 0.32                               \\
%                            & POS, Deshpande et al. \cite{deshpande2019fast}                                                                & -                                                 & 0.23                               & 0.33                               \\
%                            & Seq-CVAE, Aneja et al. \cite{Aneja2019}                                                           & -                                                 & 0.33                               & 0.48                               \\ \cmidrule(l){2-5} 
%                            & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{SeqSentiVAE   (ours)}}} & \textbf{1}                                        & \textbf{0.22}                      & \textbf{0.28}                     \\
%                            & \multicolumn{1}{c}{}                                               & \textbf{2}                                        & \textbf{0.26}                      & \textbf{0.37}                                   \\ \bottomrule
\end{tabularx}
\label{tab:results_fact_caps_div}
%\end{table}

==> tables_backup/pos_neg_joint.tex <==
\begin{table}[t]
  \centering
  \scriptsize
    \caption{Top-1 oracle scores on Senticap test split captions with positive and negative sentiments.
  $n$ denotes the number of captions generated per image.}
  \begin{tabularx}{\linewidth}{@{}Xcccccccc|ccccccc@{}}
     \toprule
            &  &\multicolumn{7}{c}{Positive} & \multicolumn{7}{c}{Negative}\\
           \cmidrule(lr){3-9} \cmidrule(lr){10-16}
     Method & $n$ & B1 & B2 & B3 & B4 & R & C & M & B1 & B2 & B3 & B4 & R & C & M\\
      
    \midrule
Senticap \cite{Mathews2015} & 1 & 49.1 & 29.1 & 17.5  & 10.8  & 36.5 & 54.4  & 16.8  & 50.0 & 31.2 & 20.3 & 13.1 & 37.9  & 61.8  & 16.8\\
StyleNet \cite{Gan2017}     & 1 & 45.3 & -- & 12.1 & -- & --& 36.3  & 12.1  & 43.7 & --  & 10.6 & --  & -- & 36.6 & 10.9  \\
You et al. \cite{You2018}   & 1 & 51.2 & 31.4 & 19.4  & 12.3  & 38.6  & 61.1 & 17.2 & 52.2 & 33.6 & 22.2 & 14.8 & 39.8 & 70.1& 17.1 \\
Chen et al. \cite{Chen2018b} & 1  & 50.5     & 30.8     & 19.1     & 12.1 & 38.0    & 60.0    & 16.6 & 50.3                            & 31.0    & 20.1 & 13.3 & 38.0  & 59.7 & 16.2    \\
Senti-Attend \cite{Nezami2018} & 1  & 57.6  & 34.2 & 20.5 & 12.7  & 45.1   & 68.6 & 18.9 & 58.6 & 35.4 & 22.3 & 14.7 & 45.7  & 71.9 & 19.0   \\
MSCap \cite{Guo2019}  & 1  & 46.9     & --   & 16.2     & --   & --  & 55.3    & 16.8 & 45.5                            & --  & 15.4  & --  & -- & 51.6  & 16.2    \\
AttendGAN \cite{Nezami2019}           & 1  & 56.9     & 33.6     & 20.3     & 12.5  & 44.3  & 61.6  &18.8& 56.2                            & 34.1 & 21.3   & 13.6  & 44.6 & 64.1 & 17.9    \\
Memcap \cite{Zhao2020}                & 1  & 51.1     & --   & 17.0     & --   & --  & 52.8    & 16.6 &49.2                   & --  & 18.1    & --  & --  & 59.4 & 15.7    \\ 
\midrule
 {Karayil   et al. \cite{Karayil2019}}  & 1   &  {54.7}   &  {34.6}  &  {22.0}   &  {14.4} &  {41.8}  &  {46.1}     &  {18.5} &   {57.0}  &  {36.2}   &  {23.4}    &  {15.1} &  {44.5}  &  {50.9} &  {19.9}  \\
 {}       & 10 &  {65.6} &  {43.9}  &  {29.5} &  {20.2}                   &  {48.8} &  {63.1} &  {22.1} &  {67.6}                   &  {46.3}                      &  {31.9}                   &  {21.9}                      &  {50.4}                     &  {68.8}                  &  {23.5} \\ 
\midrule
\multirow{2}{*}{\textbf{Senti-SeqCVAE}} & 1   & 53.8                   & {33.2}                   & {20.1}                   & {12.5}                   & {41.5}                  &  {71.1}                  & {19.7}   & {55.2}                   & {34.5}                   & {21.5}                   & {13.4}                   & {41.5}                  & {75.5}                  & {19.4}                                \\
                & 10 & \textbf{66.3}                   & \textbf{46.3}                   & \textbf{32.2}                   & \textbf{22.2}                   & \textbf{51.2}                  & \textbf{110.5}                 & \textbf{25.2}    & \textbf{66.1}                   & \textbf{46.8}                   & \textbf{33.3}                   & \textbf{23.7}                   & \textbf{50.9}                  & \textbf{111.9}                 & \textbf{24.4}   \\
              \bottomrule
  \end{tabularx}
  \smallskip
  \label{tab:senticap_baseline_joint}
  \vspace{-0.5em}
\end{table}

==> tables_backup/senticap_baseline_neg.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{\textbf{Method}}           & \multicolumn{1}{c}{\textbf{n}} & \multicolumn{1}{c}{\textbf{B1}} & \multicolumn{1}{c}{\textbf{B2}} & \multicolumn{1}{c}{\textbf{B3}} & \multicolumn{1}{c}{\textbf{B4}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{C}} & \multicolumn{1}{c}{\textbf{M}} \\ \midrule
Senticap,   Mathews et al. \cite{Mathews2015}           & 1 & 50.0                            & 31.2                            & 20.3                            & 13.1                            & 37.9                           & 61.8                           & 16.8                           \\
StyleNet, Gan   et al. \cite{Gan2017}*               & 1 & 43.7                            & -  & 10.6                            & -  & - & 36.6                           & 10.9                           \\
You et al.   \cite{You2018}                         & 1 & 52.2                            & 33.6                            & 22.2                            & 14.8                            & 39.8                           & 70.1                           & 17.1                           \\
Chen et al.   \cite{Chen2018b}                        & 1 & 50.3                            & 31.0                            & 20.1                            & 13.3                            & 38.0                           & 59.7                           & 16.2                           \\
Senti-Attend,   Nezami et al. \cite{Nezami2018}        & 1 & 58.6                            & 35.4                            & 22.3                            & 14.7                            & 45.7                           & 71.9 & 19.0\\
MSCap, Guo et   al. \cite{Guo2019}*                  & 1 & 45.5                            & -  & 15.4                            & -  & - & 51.6                           & 16.2                           \\
Attendgan,   Nezami et al. \cite{Nezami2019}           & 1 & 56.2                            & 34.1                            & 21.3                            & 13.6                            & 44.6                           & 64.1                           & 17.9                           \\
Memcap, Zhao   et al. \cite{Zhao2020}*                & 1 & 49.2                   & -                   & 18.1                   & -                   & -                  & 59.4                  & 15.7                  \\ \midrule
\textit{Karayil   et al. \cite{Karayil2019}}            & \textit{1}                     & \textit{57.0}                   & \textit{36.2}                   & \textit{23.4}                   & \textit{15.1}                   & \textit{44.5}                  & \textit{50.9}                  & \textit{19.9}                  \\
\textit{}      & \textit{10}                    & \textit{67.6}                   & \textit{46.3}                      & \textit{31.9}                   & \textit{21.9}                      & \textit{50.4}                     & \textit{68.8}                  & \textit{23.5}                  \\ \midrule
\multirow{4}{*}{\textbf{SeqSentiVAE (ours)}} & \textbf{1}                     & \textbf{55.2}                   & \textbf{34.5}                   & \textbf{21.5}                   & \textbf{13.4}                   & \textbf{41.5}                  & \textbf{75.5}                  & \textbf{19.4}                  \\
               & \textbf{5}                     & \textbf{63.9}                   & \textbf{43.8}                   & \textbf{30.2}                   & \textbf{20.8}                   & \textbf{48.5}                  & \textbf{101.7}                 & \textbf{23.2}                  \\
               & \textbf{10}                    & \textbf{66.1}                   & \textbf{46.8}                   & \textbf{33.3}                   & \textbf{23.7}                   & \textbf{50.9}                  & \textbf{111.9}                 & \textbf{24.4}                  \\
               & \textbf{100}                   & \textbf{74.0}                   & \textbf{56.3}                   & \textbf{43.1}                   & \textbf{33.0}                   & \textbf{57.9}                  & \textbf{145.8}                 & \textbf{28.7}                  \\ \bottomrule
\end{tabular}
\caption{Top-1-Oracle scores on Senticap test split captions with negative sentiment.}
\label{tab:senticap_baseline_neg}

==> tables_backup/senticap_baseline_pos.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}

\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{\textbf{Method}}           & \multicolumn{1}{c}{\textbf{n}} & \multicolumn{1}{c}{\textbf{B1}} & \multicolumn{1}{c}{\textbf{B2}} & \multicolumn{1}{c}{\textbf{B3}} & \multicolumn{1}{c}{\textbf{B4}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{C}} & \multicolumn{1}{c}{\textbf{M}} \\ \midrule
Senticap,   Mathews et al. \cite{Mathews2015}           & 1                              & 49.1                            & 29.1                            & 17.5                            & 10.8                            & 36.5                           & 54.4                           & 16.8                           \\
StyleNet, Gan   et al. \cite{Gan2017}*               & 1                              & 45.3                            & -                               & 12.1                            & -                               & -                              & 36.3                           & 12.1                           \\
You et al.   \cite{You2018}                         & 1                              & 51.2                            & 31.4                            & 19.4                            & 12.3                            & 38.6                           & 61.1                           & 17.2                           \\
Chen et al.   \cite{Chen2018b}                        & 1                              & 50.5                            & 30.8                            & 19.1                            & 12.1                            & 38.0                           & 60.0                           & 16.6                           \\
Senti-Attend,   Nezami et al. \cite{Nezami2018}        & 1                              & 57.6                            & 34.2                            & 20.5                            & 12.7                            & 45.1                           & 68.6                           & 18.9                           \\
MSCap, Guo et   al. \cite{Guo2019}*                  & 1                              & 46.9                            & -                               & 16.2                            & -                               & -                              & 55.3                           & 16.8                           \\
Attendgan,   Nezami et al. \cite{Nezami2019}           & 1                              & 56.9                            & 33.6                            & 20.3                            & 12.5                            & 44.3                           & 61.6                           & 18.8                           \\
Memcap, Zhao   et al. \cite{Zhao2020}*                & 1                              & 51.1                            & -                               & 17.0                            & -                               & -                              & 52.8                           & 16.6                           \\ \midrule
\textit{Karayil   et al. \cite{Karayil2019}}            & \textit{1}                     & \textit{54.7}                   & \textit{34.6}                   & \textit{22.0}                   & \textit{14.4}                   & \textit{41.8}                  & \textit{46.1}                  & \textit{18.5}                  \\
\textit{}                                   & \textit{10}                    & \textit{65.6}                   & \textit{43.9}                   & \textit{29.5}                   & \textit{20.2}                   & \textit{48.8}                  & \textit{63.1}                  & \textit{22.1}                  \\ \midrule
\multirow{4}{*}{\textbf{SeqSentiVAE (ours)}} & \textbf{1}                     & \textbf{53.8}                   & \textbf{33.2}                   & \textbf{20.1}                   & \textbf{12.5}                   & \textbf{41.5}                  & \textbf{71.1}                  & \textbf{19.7}                  \\
                                            & \textbf{5}                     & \textbf{63.4}                   & \textbf{43.5}                   & \textbf{29.5}                   & \textbf{19.9}                   & \textbf{49.0}                  & \textbf{99.2}                 & \textbf{23.9}                  \\
                                            & \textbf{10}                    & \textbf{66.3}                   & \textbf{46.3}                   & \textbf{32.2}                   & \textbf{22.2}                   & \textbf{51.2}                  & \textbf{110.5}                 & \textbf{25.2}                  \\
                                            & \textbf{100}                   & \textbf{73.2}                   & \textbf{54.8}                   & \textbf{41.5}                   & \textbf{31.6}                   & \textbf{57.6}                  & \textbf{141.8}                 & \textbf{29.0}                  \\ \bottomrule
\end{tabular}
\caption{Top-1-Oracle scores on Senticap test split captions with positive sentiment: Performance according to each metric in comparison to work in the same domain. The column "n" is the number of generated samples. For the caption quality metrics, "B" is short for BLEU, "R" for ROUGE-L, "C" for CIDEr-D, "M" for METEOR. Approaches marked with "*" are multi style captioning approaches. Thus, a direct comparison is unfair, but for the sake of completeness they are included. Evaluation scores on a subset of the original test split are shown in italics. However, comparisons have shown that scores achieved on this subset are very similar to the full evaluation.}
\label{table:senticap_baseline_pos}

==> tables_backup/senticap_baseline_senti_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\scriptsize
\centering
\caption{Additional evaluation on the Senticap test set. SP denotes the sentiment precision and SR the sentiment recall.}
\begin{tabularx}{\textwidth}{cXrrrrrrrrrr}
\toprule
\textbf{n}          & \multicolumn{1}{c}{\textbf{Method}}      & \multicolumn{1}{c}{\textbf{B1}} & \multicolumn{1}{c}{\textbf{B2}} & \multicolumn{1}{c}{\textbf{B3}} & \multicolumn{1}{c}{\textbf{B4}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{C}} & \multicolumn{1}{c}{\textbf{M}} & \multicolumn{1}{c}{\textbf{\%SEN}} & \multicolumn{1}{c}{\textbf{SP}} & \multicolumn{1}{c}{\textbf{SR}} \\ \midrule
\multirow{3}{*}{1}  & Senticap,   Mathews et al. \cite{Mathews2015}                                 & 48.8                            & 29.8                            & 18.7                            & 11.8                            & 37.2                           & 56.6                           & 16.8                           & 87.5                              & 0.33                                  & 0.14                                 \\
                    & COCO + Senticap-augm.              & 54.5                            & 33.9                            & 20.8                            & 13.0                            & 41.5                           & 73.3                           & 19.6                           & 93.6                              & 0.30                                  & 0.15                                 \\
                    & COCO + Senticap-augm. + CBS & 54.7                            & 34.0                            & 21.1                            & 13.2                            & 41.7                           & 74.1                           & 19.7                           & 100.0                             & 0.30                                  & 0.15                                 \\
                   % & COCO + 20xSenticap + constr.        & 55.8                            & 35.1                            & 22.2                            & 13.9                            & 41.8                           & 74.2                           & 18.7                           & 100.0                             & 0.30                                  & 0.1                                  \\ 
                   \midrule
\multirow{2}{*}{10} & COCO + Senticap-augm.              & 66.2                            & 46.6                            & 32.8                            & 23.0                            & 51.0                           & 111.2                          & 24.8                           & 99.3                              & 0.26                                  & 0.30                                 \\
                    & COCO + Senticap-augm. + CBS & 66.3                            & 47.2                            & 33.6                            & 23.9                            & 51.5                           & 114.5                          & 25.3                           & 100.0                             & 0.25                                  & 0.32                                 \\
                    %& COCO + 20xSenticap + constr.        & 68.4                            & 48.2                            & 34.2                            & 24.2                            & 51.4                           & 115.9                          & 25.0                           & 100.0                             & 0.23                                  & 0.31                                 \\ 
                    \bottomrule
\end{tabularx}
\label{tab:results_sentiment_metrics}
\vspace{-0.5em}
\end{table}

==> tables_backup/swd_vs_glove.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htb]
\centering
\footnotesize
\begin{tabular}{ccrrrrr}
\hline
\multirow{2}{*}{\textbf{n}} & \multirow{2}{*}{\textbf{Method}}                                           & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{std}}} & \multicolumn{2}{c}{\textbf{n-gram Diversity}}                           & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Top-1\\ C\end{tabular}}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Avg\\ C\end{tabular}}}} \\ \cline{4-5}
                            &                                                                            & \multicolumn{1}{c}{}                              & \multicolumn{1}{c}{\textbf{Div-1}} & \multicolumn{1}{c}{\textbf{Div-2}} & \multicolumn{1}{c}{}                                                                            & \multicolumn{1}{c}{}                                                                          \\ \hline
                            & \multirow{2}{*}{Basic}                                                     & 1                                                 & 0.27                                  & 0.39                                  & 137.4                                                                                               & 78.3                                                                                             \\
                            &                                                                            & 2                                                 & 0.34                                  & 0.55                                  & 131.1                                                                                               & 61.6                                                                                             \\ \cline{2-7} 
20                          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}SeqSentiVAE\\ SWD\end{tabular}} & 1                                                 & 0.27                               & 0.39                               & 137.9                                                                                           & 78.9                                                                                          \\
                            &                                                                            & 2                                                 & 0.34                               & 0.55                               & 130.5                                                                                           & 60.8                                                                                          \\ \cline{2-7} 
                            & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}SeqSentiVAE\\ ATT\end{tabular}} & 1                                                 & 0.23                               & 0.31                               & 130.4                                                                                           & 84.9                                                                                          \\
                            &                                                                            & 2                                                 & 0.29                               & 0.43                               & 137.2                                                                                           & 75.2                                                                                          \\ \hline
                            & \multirow{2}{*}{Basic}                                                     & 1                                                 & 0.25                                  & 0.34                                  & 157.2                                                                                               & 78.5                                                                                             \\
                            &                                                                            & 2                                                 & 0.31                                  & 0.48                                  & 158.6                                                                                               & 61.5                                                                                             \\ \cline{2-7} 
100                         & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}SeqSentiVAE\\ SWD\end{tabular}} & 1                                                 & 0.25                               & 0.34                          & 157.6                                                                                        & 78.8                                                                                             \\
                            &                                                                            & 2                                                 & 0.31                               & 0.48                                  & 157.9                                                                                               & 60.7                                                                                             \\ \cline{2-7} 
                            & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}SeqSentiVAE\\ ATT\end{tabular}} & 1                                                 & 0.22                               & 0.28                               & 144.7                                                                                           & 85.0                                                                                          \\
                            &                                                                            & 2                                                 & 0.26                               & 0.37                               & 158.8                                                                                           & 75.0                                                                                          \\ \hline
\end{tabular}
\caption{Comparison of different latent space structuring approaches.}
\label{tab:my-table}
\end{table}
